Interpretable Machine Learning Models for Modal Split Prediction in Transportation Systems

Modal split prediction in transportation networks has the potential to support network operators in managing traffic congestion and improving transit service reliability. We focus on the problem of hourly prediction of the fraction of travelers choosing one mode of transportation over another using high-dimensional travel time data. We use logistic regression as base model and employ various regularization techniques for variable selection to prevent overfitting and resolve multicollinearity issues. Importantly, we interpret the prediction accuracy results with respect to the inherent variability of modal splits and travelers' aggregate responsiveness to changes in travel time. By visualizing model parameters, we conclude that the subset of segments found important for predictive accuracy changes from hour-to-hour and include segments that are topologically central and/or highly congested. We apply our approach to the San Francisco Bay Area freeway and rapid transit network and demonstrate superior prediction accuracy and interpretability of our method compared to pre-specified variable selection methods.

==> responsiveness.tex <==
\section{Statistical Tests}\label{sec:responsiveness}

The first method for quantifying responsiveness is the F-test, a statistical fit test for regression models trained following the methods presented in Sec. \ref{sec:method}. The second method is an analysis of the correlation between travel times for individual segments and aggregate driving flow. The key distinction between these two analyses is that the F-test yields results for the regression model as a whole while the correlation analysis results are aggregated segment-by-segment.

\subsection{F-Test}
For all methods described in Sec. \ref{sec:method}, we test the significance of the model fit using an F-test. Specifically, we want to determine if the driving fraction depends on the driving travel times by testing the hypothesis
\begin{align*}
    H_0: \beta = 0, \hspace{5mm} H_1: \beta \neq 0,
\end{align*}
or that the true parameters are zero. Given the mean observed driving fraction, $\overline{Y}_t$, we calculate the F statistic as
\begin{align*}
    F = \frac{\left(\frac{\text{RSS}_1-\text{RSS}_2}{\nu-1}\right)}{\left(\frac{\text{RSS}_2}{n-\nu}\right)}
\end{align*}
where $\text{RSS}_1$ and $\text{RSS}_2$ are
\begin{align*}
    \text{RSS}_1 &= \sum_{j=1}^{n} \left(\log\left(\frac{1}{Y_t^{(j)}}-1\right) - \log\left(\frac{1}{\overline{Y}_t - 1}\right)\right)^2 \\
    \text{RSS}_2 &= \sum_{j=1}^{n} \left(\log\left(\frac{1}{Y_t^{(j)}}-1\right) - \phi_i\left(X_t^{(j)},...,X_{t-k\delta}^{(j)}\right)\right)^2.
\end{align*}

$F$ is distributed according to an F-distribution with ${(\nu-1, n-\nu)}$ degrees of freedom. We reject the null hypothesis at a significance level of $\alpha$ if ${F > F_\alpha(\nu-1,n-\nu)}$. Here, $\nu < |N|(k+1)$ denotes the number of degrees of freedom in our estimated model -- a measure of the model complexity -- which is calculated differently for each of the methods described in Sec. \ref{sec:method}. For Betweenness Selection, Congestion Selection, and LASSO Regression, $\nu$ is equal to the number of non-zero coefficients. For Ridge Regression, $\nu$ is calculated as $\text{Trace}(\mathcal{X}_t(\mathcal{X}_t'\mathcal{X}_t+\lambda_t I)^{-1}\mathcal{X}_t')$ given the regularization penalty $\lambda_t$. For PCR, $\nu$ is equal to $L_t$, the number of principal components.

The responsiveness of aggregate driving fraction to changes in travel time in each time period can again be characterized using the F-test results. A low $p$-value (i.e. highly significant model fit) indicates high responsiveness of driving fraction to travel times in the respective time period.

\subsection{Correlation Analysis}
We denote by $\text{Corr}\left(Y_t, X_{t-i\delta}^{(j)}\right) \in [0,1]$ the correlation of the observed travel time of segment $j$ in time $t-i\delta$ with $Y_t$, the aggregate driving fraction in time $t$. For each time period $t$, we average the correlation coefficients across all time lags to yield
\begin{align*}
    \overline{\text{Corr}}\left(Y_t, X_t^{(j)}\right) = \frac{1}{k+1} \sum_{i=0}^k \text{Corr}\left(Y_t, X_{t-i\delta}^{(j)}\right)
\end{align*}
for all segments $j=1,\dots,|N|$. Highly negative values of $\overline{\text{Corr}}\left(Y_t, X_t^{(j)}\right)$ suggest that high travel times for freeway segment $j$ are highly correlated with decreased demand for driving, and consequently, travelers decisions are more responsive to changes in travel time on segment $j$.

In Sec. \ref{sec:empirical}, we aggregate these correlations across all segments $j=1,\dots,|N|$ and plot a responsiveness function $g_t(\rho):[0,1] \to \mathbb{Z}$ defined as
\begin{align*}
    g_t(\rho) = \Big|\Big\{\overline{\text{Corr}}\left(Y_t, X_t^{(j)}\right) \mid \overline{\text{Corr}}\left(Y_t, X_t^{(j)}\right) < \rho \hspace{3mm} \forall j\Big\}\Big|.
\end{align*}
Intuitively, this function maps a given correlation threshold, $\rho\in [0,1]$, to the number of segments in the network with an average correlation $\overline{\text{Corr}}\left(Y_t, X_{t-i\delta}^{(j)}\right)$ less than $\rho$. This is a monotonic increasing function of $\rho$ bounded between $0$ and $|N|$. The motivation for plotting these function is to visually compare the relative responsiveness of aggregate flows to changes in driving time across different hours.
